Energy Predictive Models with Limited Data using Transfer Learning

In this paper, we consider the problem of developing predictive models with limited data for energy assets such as electricity loads, PV power generations, etc. We specifically investigate the cases where the amount of historical data is not sufficient to effectively train the prediction model. We first develop an energy predictive model based on convolutional neural network (CNN) which is well suited to capture the interaday, daily, and weekly cyclostationary patterns, trends and seasonalities in energy assets time series. A transfer learning strategy is then proposed to address the challenge of limited training data. We demonstrate our approach on a usecase of daily electricity demand forecasting. we show practicing the transfer learning strategy on the CNN model results in significant improvement to existing forecasting methods.

==> Sections/Abstract.tex <==
\begin{abstract}

In this paper, we consider the problem of developing predictive models with limited data for energy assets such as electricity loads, PV power generations, wind turbines production, etc. We specifically investigate the cases where the amount of historical data is not sufficient to effectively train the prediction model. We first develop an energy predictive model based on convolutional neural network (CNN) which is well suited to capture the interaday, daily, and weekly cyclostationary patterns, trends and seasonalities in energy assets time series. A transfer learning strategy is then proposed to address the challenge of limited training data. We demonstrate our approach on a usecase of daily electricity demand forecasting. Through a comprehensive simulation studies on 23 commercial and industrial customers in different categories such as school, grocery, manufacturing, hospital, bank, etc., we show practicing the transfer learning strategy on the CNN model results in significant improvement to existing forecasting methods.

Keyword: Energy analytics, predictive models, time series, transfer learning, convolutional neural network (CNN), daily electricity load forecasting. 

\end{abstract}


==> Sections/LoadForecasting.tex <==
\section{Problem of Electricity Load Forecasting}\label{sec:LoadForecasting}

In this section, we describe the problem of electricity load forecasting for demand charge minimization applications and propose our approach of conditioning the load forecasting model with the demand charge computation module. 

\subsection{Background}

A commercial and industrial (C\&I) type electricity bill includes two main components, namely energy and demand charges~\cite{pge}. The energy component shows the amount of energy (kilo Watt hour) consumed by the customer during a billing period that is typically a month. The demand charge (DC) is calculated based on the highest power demand (kilo Watt), which is measured at the meter (point of connection to the power grid) during the same billing period. The demand charge is a significant portion of the bill (up to half of the total monthly charges~\cite{oudalov2007sizing}). 


In order to reduce the demand charge, customers deploy behind-the-meter (BTM) energy storage systems, so that when the demand is high, the power is provided by battery rather than the electrical grid~\cite{moslemi2017data, moslemi2017machine}. Fig.~\ref{fig:DCT} shows an example daily demand and the battery operation. The figure shows that a storage solution is employed from 9:00 to 14:00 when the customer experiences its peak demand. Using the storage reduces the peak demand read at the meter and consequently reduces the demand charge. After 14:00, battery is charged to be prepared for the next peak demand event.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{Figures/DCT.pdf}
	\caption{An example of daily battery operation for the application of demand charge minimization. A storage solution is employed from 9:00 to 14:00 when the customer experiences its peak demand. After 14:00, battery is charged to be prepared for the next peak demand event. Using the storage reduces the peak demand read at the meter and consequently reduces the demand charge.}
	\label{fig:DCT}
\end{figure}


To utilize the battery efficiently and minimize the demand peak, a control module is deployed to determine the charging schedule of the storage system in a way that battery is charged during off-peak periods of the load profile and discharged during peak periods. To do so, the control module computes a threshold, called Demand Charge Threshold (DCT), below which the battery is charged and otherwise discharged. The threshold is the minimum value for which after using the battery, the peak demand will never exceed it. The DCT computation problem is stated as follows:
\begin{align}
DCT = &\min_{p, s} \max_{t\in[1,T]} (x_t + p_t) \label{eq:min}\\
\nonumber\mbox{s.t. } 
&|p_t| \leq p_{\max},\\
\nonumber&s_t = s_{t-1} + p_t\Delta t, \\
\nonumber&0\leq s_t \leq C.
\end{align}
where $\{x_t\}_{t=1,\cdots,T}$ denotes the time-series data of electrical consumption and $p_t$ is the battery charging or discharging power. The battery State of Charge (SoC) at time $t$ is denoted by $s_t$ and the initial SoC is $s_0$. Battery capacity is denoted by $C$ and $p_{\max}\Delta t$ is the maximum energy that battery can be charged/discharged in time duration $\Delta t$.

\subsection{Demand Charge-Aware Load Forecasting}

DCT computation algorithm takes load profile and battery parameters as inputs and outputs the optimal DCT. The DCT value must be set at the beginning of each billing cycle. Therefore, the optimization problem should be solved with forecast values of load profile. The DCT value obtained from Equ.~\ref{eq:min} is sensitive to errors in load forecasting. As a result, the demand charge management system usually experiences DCT under- or overestimations. In the case of DCT overestimation, the battery is not fully utilized, which results in inefficient peak shaving. DCT underestimation causes the battery to deplete in the middle of a major peak, resulting in higher values of demand peak and thus losing the demand charge savings. 

Existing techniques for electricity forecasting typically provide a prediction that on average matches the actual values, while smoothing the peaks. 
For the application of demand charge minimization, we need a method that forecasts the load in such a way that the resultant DCT matches the DCT of the actual load. We call such method {\it demand charge-aware load forecasting}. 
Figure~\ref{fig:example} illustrates the importance of accounting for demand charge when forecasting the load, by showing  an example load and two different forecasts. While forecast $2$ is better in terms of mean absolute error (MAE) minimization, forecast $1$ is much better when used for the application of demand charge minimization, because it could better approximate the shape of the actual load. 



\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{Figures/TwoForecasts.pdf}
	\caption{An illustration of the importance of accounting for demand charge minimization when forecasting the load. An example load and two different load forecasts are shown. Shaded area shows the times where forecast $2$ is closer to actual load compared to forecast $1$. While forecast $2$ is better in terms of mean absolute error (MAE) minimization, forecast $1$ is much better when used for the application of demand charge minimization, because it could better approximate the shape of the actual load.}
	\label{fig:example}
\end{figure}


\subsection{Our Approach: Conditional Load Forecasting}

In this section, we propose a demand charge-aware load forecasting method. 
Figure~\ref{fig:overall} shows the block diagram of the model. The load forecast module is followed by the DCT computation module and is updated in such a way that the forecast load performs well when used for computing the optimal DCT value. 

Let $F_{\theta}$ be a machine learning model with parameters $\theta$ used for load forecasting and $g$ be the DCT computation module. 
The problem of demand charge-aware load forecasting is stated as follows:
\begin{align}\label{eq:aware}
\min_{\theta} \|y-F_{\theta}(x)\| + \lambda |g(y) - g(F_{\theta}(x))|
\end{align}
where $x$ is the historical data and $y$ is the load profile to be predicted. 
The DCT computation module, however, cannot be expressed in closed form. Therefore, we cannot determine how $\theta$ must be updated to reduce the second term in the loss function. As discussed in Section~\ref{sec:condition} and shown in Fig.~\ref{fig:train}, we replace the DCT computation module with a learned conditioner. 
That is, we train the model with two outputs of load profile and its corresponding DCT. The entire model is trained end-to-end. The revised learning problem is stated as follows:
\begin{align}\label{eq:learned}
\min_{\theta} \|y-F_{\theta}(x)\| + \lambda |g(y) - \hat{g}(F_{\theta}(x))|.
\end{align}
The component $\hat{g}$ is essentially approximating the DCT optimization module. It thus forces the first component to forecast the load in such a way that the error in DCT is also minimized. 

As explained in Fig.~\ref{fig:method}, at test time, we only use the load forecasting model in the demand charge management pipeline. The optimal DCT of the forecast load is computed using the original optimization problem~\ref{eq:min}, since it provides the exact results. 


\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{Figures/Overall.pdf}
	\caption{Block diagram of the demand charge-aware load forecasting method.}
	\label{fig:overall}
\end{figure}

==> Sections/Related.tex <==
\section{Related Works}

Several papers have proposed methods for reducing the demand charge by using behind-the-meter battery solutions~\cite{alt1997assessment, lu2014optimal,yang2014sizing}. One straightforward approach for efficient scheduling of battery charging/discharging is to set a predetermined demand charge threshold (DCT) for the entire billing period. This approach is easy to implement and does not require monitoring infrastructures~\cite{hida2010load}. The optimal DCT value is obtained by solving an optimization problem that takes the load profile as input. 
However, due to the sensitivity of DCT computation function to the input load, the forecasting errors cause the estimated DCT to significantly deviate from the optimal value~\cite{moslemi2017machine}. 

In this paper, we proposed to jointly minimize the error in forecast load and its corresponding DCT, by replacing the DCT computation module with a learned model. We showed that the proposed approach significantly reduces the error in DCT estimation without losing accuracy on load forecasting. 


Model conditioning can be considered in the context of generative adversarial networks (GAN)~\cite{goodfellow2014generative}, where the generator is conditioned to generate images that look ``natural.'' Compared to the GAN problem, we require the main model to minimize a loss function of its own, in addition to satisfying the requirements of the conditioner. Moreover, we assume that the conditioner is a known function which we have black-box access to. Therefore, unlike the discriminator model in GAN framework, the ground-truth for the output of the learned conditioner is obtained by querying the original conditioner. 


Deep learning models are widely deployed for time-series forecasting~\cite{schmidhuber2015deep}. Several papers have adopted such techniques in power system applications~\cite{busseti2012deep,wang2017deep}. In this paper, we used a convolutional neural network (CNN) to forecast electricity load profile of the next day. We proposed to reshape historical electricity data into a three dimensional matrix. The matrix is formed in such a way that it exhibits local correlations across every axis corresponding to hourly, daily and weekly correlations. We chose the CNN model over Recurrent Neural Networks (RNN), since it can efficiently extract correlations in electricity usages at different time-scales. Several other papers have also reported case-studies where CNNs outperform RNNs for time-series data~\cite{lee2009unsupervised,kalchbrenner2014convolutional,bai2018empirical}. 



Many real-world tasks involve learning from multiple data sources and generating multiple outputs. Data can be of different natures and modalities, e.g., images, categorical data of different types, time-series data, etc.
Typical machine learning models take one source of input and generate one output. 
However, a class of problems that involve processing two inputs has gained attention recently~\cite{dumoulin2018feature-wise}. %For example, visual question-answering task involves answering compositional questions about synthetic images. Also, style transfer is used to transfer the input image into the given style~\cite{}. 

Our proposed model takes multiple inputs and generates two outputs. We exploited the problem domain knowledge to develop a customized model structure in such a way that it efficiently learns the dependencies between variables. For example, we used auxiliary inputs of customer index and pattern of holidays to weight the features extracted by the convolutional network. We also used the battery parameters as input to the final component, since that input is only needed by the DCT computation module. Our model is designed to be interpretable in terms of the relationships between variables and can be easily extended for further applications and/or integrated in larger modules. 




%Battery technologies are an essential constituent for future energy needs and have gained a lot of attention from power system community~\cite{koohi2013emergence, zhang2008application, wang2013review}. Due to the unprecedented growth in capacities, batteries are proved to be a vital component for a wide range of applications including integration with renewable generations, electric vehicles, frequency regulation systems, voltage support, behind and front the meter services, microgrids, etc~\cite{hooshmand2013power, tie2013review, khaligh2010battery, kempton2008test, kottick1993battery, liu2012coordinated, hooshmand2012predictive, zamora2010controls}. 

%Battery operations are controlled by an Energy Management Systems (EMS)~\cite{hooshmand2014experimental, hooshmand2017multi}. 
%EMS managed storage devices are commonly deployed by behind-the-meter (BTM) commercial and industrial (C\&I) customers for the two purposes of increasing renewable utilization and reducing their demand charge, as depicted in Fig.~\ref{fig:1}. 
%For the first case, storage device helps C\&I customers to maximize the local consumption of their uncontrollable renewable generation (mostly solar generations) to reduce electricity bill charges. 
%For the second use case, storage device helps to reduce the electricity bills by shaving peak electrical demand, as explained in the following.
%Battery device helps to minimize the DC by supplying the electrical demand during the peak hours~\cite{moslemi2017data, moslemi2017machine}.





